Electromagnetic calorimeter simulation for future $\mu \to e$ conversion experiments

We examine three dense high-Z scintillating crystals for the $\mu \to e$ conversion experiment using the GEANT4 simulation toolkit. The full energy deposition, albedo, and longitudinal and lateral energy leakages for all crystal assemblies are studied. The influence of the crystal depth on the energy deposition in the calorimeter is studied.

==> edepleak_width.tex <==
%%%%%\vspace*{-3cm}    
\begin{table}[]
\large { \vspace {-2.3cm}
\begin{center}
{\color{black}        
\begin{tabular}{||c||c||c||c||c||}     \hline \hline
Crystal   &                     &                 &                      &               \\              
depth (cm)&$E_{dep}(MeV)       $& Albedo (MeV)    & Longitudinal(MeV)    & Lateral(MeV)  \\ \hline \hline              
          &98.27               &0.962             &3.584             &1.879      \\                   
 8.0      &4.142               &1.227             &5.816             &1.416      \\
          &50000               &40555             &160816            & 191       \\ \hline
          &99.23               &0.9677            &3.409             &1.984      \\                   
 9.0      &4.105               &1.221             &5.411             &1.524      \\
          &50000               &40738             &127695            &227        \\ \hline
          &101.1               &0.9587            &3.322             &1.832      \\                   
 10.0     &4.008               &1.215             &5.108             &1.553      \\
          &50000               &40665             &100658            & 276       \\ \hline          
          &100.8               &0.9591            &3.196             &1.883      \\                   
 11.0     &3.854               &1.213             &4.824             &1.701      \\
          &50000               &40845             &79339             & 310       \\ \hline         
          &101.5               &0.9653            &3.156             &1.852       \\                   
 12.0     &3.618               &1.227             &4.685             &1.447       \\
          &50000               &40739             &61835             & 331         \\ \hline         
          &102.0               &0.9819            &3.12              &1.988        \\                   
 13.0     &3.388               &1.257             &4.481             &1.873       \\
          &50000               &40627             &49502             & 348        \\ \hline \hline         
\end {tabular}
\caption{ Energy deposition, albedo, lonitudinal and lateral energy leakages for LYSO(Ce)   
and different crystal depth.}
}
\end{center}
}
\end{table}


